Designing Personalized Interaction of a Socially Assistive Robot for Stroke Rehabilitation Therapy

The research of a socially assistive robot has a potential to augment and assist physical therapy sessions for patients with neurological and musculoskeletal problems (e.g. stroke). During a physical therapy session, generating personalized feedback is critical to improve patient's engagement. However, prior work on socially assistive robotics for physical therapy has mainly utilized pre-defined corrective feedback even if patients have various physical and functional abilities. This paper presents an interactive approach of a socially assistive robot that can dynamically select kinematic features of assessment on individual patient's exercises to predict the quality of motion and provide patient-specific corrective feedback for personalized interaction of a robot exercise coach.

==> contents/intro.tex <==
\section{Introduction}
Stroke is the leading cause of disability and the most common neurological disorder worldwide \cite{feigin2017global}. An early and extensive physical therapy session with task-oriented exercises is an effective intervention for post-stroke subjects to regain their functional ability \cite{o2019physical}. However, post-stroke survivors can receive only limited amount of those supervised sessions due to the costs and the shortage of therapists.
%Although physical therapy sessions are critical process to regain functionality of a post-stroke patient with neurological and musculoskeletal problems, post-stroke survivors can receive only limited amount of those supervised sessions due to the costs and the shortage of therapists.

Recent advance in computing and artificial intelligence empowers a robot with various autonomous capabilities to understand and interact with the world \cite{hirschberg2015advances}. Researchers have explore the possibility of supplementing health services with advanced computing \cite{webster2014systematic} and socially assistive robotics (SAR) \cite{feil2005defining}. For instance, researchers envision that a SAR can be integrated into the rehabilitation process by automatically monitoring patient's exercise and providing motivation on patient's in-home rehabilitation until patient's next visits to a therapist \cite{mataric2007socially}. Prior work demonstrates that the physical embodiment of a robot is considered more effective and acceptable for elderly people than the virtual robot embodiment \cite{fasola2013socially}. Elderly or post-stroke subjects can successfully exercise and stay engaged with a robot over a single \cite{swift2015effects} or multiple sessions \cite{gorer2017autonomous}. 

%revealed that elderly people can successfully exercise with the assistance of the robot, while staying engaged with the system over multiple sessions.
In spite of this potential, prior work is limited to provide pre-defined corrective feedback on patient's exercise performance (e.g. angular difference with a motion template \cite{fasola2013socially,gorer2017autonomous}), which is fixed over all subjects. Generating tailored feedback for an individual still remain a challenge \cite{gorer2017autonomous}. 




%suser adherence on patient's exercise
%and provide motivation and support on patient's in-home rehabilitation exercises until patient's next visits to a therapist.
%Researchers envision that a SAR can be integrated in 
%A Socially Assistive Robot (SAR) can be integrated into the rehabilitation process to provide motivation and support through social interaction for at-home or self-directed in-clinic rehabilitation exercises between visits to an occupational or physical therapist.
%For instance, a SAR can monitor exercise motions of a post-stroke subject and provide audio-based verbal feedback 
%monitor exercise motions of a post-stroke subject and provide audio-based verbal feedback.

%In accordance with the vision of successful aging, we describe in this study an autonomous robotic exercise tutor for elderly people. The robot learns a set of physical exercises from a human demonstrator in an imitation framework, and performs these motions in an exercise scenario, while monitoring the elderly person to provide verbal feedback.


%that support health and wellness through co-presence and social interaction.
%robotics \cite{feil2005defining}. 
%The field of socially assistive robotics (SAR) is to develop a robotic system that support health and wellness through co-presence and social interaction \cite{feil2005defining}.



%have social capacity of a robot to  

In this paper, we presents an approach of motion analysis that can automatically identify the most salient features for assessment to predict the quality of motion and generate personalized corrective feedback. 
%Building upon the prior work on creating a rehabilitation assessment system \cite{Lee2019LAQ}, 
this paper presents an interactive assistive robot (Figure \ref{fig:flow-diagram}) that can automatically identify salient features for assessment and predict the quality of motion. Utilizing identified kinematic features and user's held-out normal motions, a robot can analyze which kinematic variables have been deviated from normal motions, and generate audio-based real-time feedback on a patient's exercise motion (Figure \ref{fig:web-interface}). In future, this interactive personalized assessment will be deployed to a socially assistive robot \cite{shamsuddin2012initial} and post-stroke survivors will be recruited to conduct a study whether the presented interactive assistive robot with personalized corrective feedback can enhance user's engagement to participate in rehabilitation exercises. 

%This paper presents an interactive machine learning technique to derive personalized behavior analysis and interactions for elderly care robots (Fig. \ref{figures:flow-diagram-iml}). This technique utilizes only few demonstrations/samples to define the goal of a user (e.g. normal behaviour sequences or correct exercise motions) and identify contextual features (e.g. the time/frequency of an activity or joint positions) that has been deviated from the goal \cite{Lee2019IAAG}. Based on the identified contextual features, a robot can explain behaviour analysis of machine learning models to derive transparent interaction \cite{amershi2019guidelines}. In addition, a robot can elicit human feedback (e.g. generating dialogue responses or rules to monitor physical status) for personalized analysis and interaction. 

\begin{comment}
\begin{figure*}[tp!]
\centering
\begin{subfigure}[t]{.4\textwidth}
\centering
  \includegraphics[width=1.0\columnwidth]{figures/flow.png}
  \caption{}
  \label{fig:flow-diagram}
\end{subfigure}\hfill
\begin{subfigure}[t]{.6\textwidth}
  \centering
  \includegraphics[height=0.3\columnwidth]{figures/setup-together.png}
  \caption{}
  \label{fig:web-interface}
\end{subfigure}
    \caption{(a) Flow diagram of a Socially Assistive Robot for Personalized Stroke Rehabilitation Therapy. (b) Figure on the left describes the setup of a system with a Kinect sensor, a tablet with the interface, the NAO robot. Figure on the right indicates an example of rehabilitation assessment with corrective feedback.}
\end{figure*}
\end{comment}

\begin{figure*}[tp!]
\centering
\begin{subfigure}[t]{.4\textwidth}
\centering
  \includegraphics[width=1.0\columnwidth]{figures/flow.png}
  \caption{}
  \label{fig:flow-diagram}
\end{subfigure}
\begin{subfigure}[t]{.2\textwidth}
  \centering
  \includegraphics[height=0.9\columnwidth]{figures/setup-robot.png}
  \caption{}
  \label{fig:web-interface}
\end{subfigure}
\begin{subfigure}[t]{.35\textwidth}
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/setup-feedback.png}
  \caption{}
  \label{fig:web-interface}
\end{subfigure}
    \caption{(a) Flow diagram of an interactive approach for an assistive robot during physical therapy. (b) the setup of a system with a Kinect sensor, a tablet with the visualization interface, the NAO robot. (c) An example output of the visualization interface that presents assessment of patient's exercise performance with corrective feedback.}
\end{figure*}

\section{Interactive Assistive Robot for Personalized Rehabilitation Assessment} \label{sect:monitor-exercise}


It is questionable how to select kinematic variables for assessment and how well a robot can provide personalized assessment of a patient's rehabilitation exercise. 
If a robot just notifies the output of pre-defined corrective feedback, a patient might consider a robot as not useful and reject to interact with it more \cite{pain2007readiness}. Thus, it is critical to derive a personalized assessment model of a robot for physical therapy sessions. 


Even if prior work demonstrated the feasibility of automatically assessing rehabilitation exercises \cite{Lee2019LAQ}, it is challenging to replicate therapist's assessment. In addition, simply presenting the predicted assessment on patient's rehabilitation performance is not convincing to a user. This work aims to support a transparent interaction between a system and user with a sparse model by feature selection \cite{biran2017explanation}. Specifically this paper applies reinforcement learning to identify salient feature for assessment. Utilizing an identified kinematic features, this approach predict the quality of motion and generate personalized corrective feedback with held-out user's normal motions (Figure \ref{fig:web-interface}). 

For identifying salient features of assessment, this paper utilizes Reinforcement Learning with Double Q-learning \cite{van2016deep} to train an agent that sequentially decides whether another feature is necessary to assess an exercise while receiving a negative reward for requesting an additional feature. For Prediction Model (PM), Neural Network (NN) is trained for the prediction model while grid-searching various architectures (i.e. one to three layers with 32, 64, 128, 256, 512 hidden units) and learning rates (i.e. $0.0001, 0.005, 0.001, 0.01, 0.1$) using \textit{`PyTorch'} libraries \cite{paszke2017automatic}. \textit{`ReLu'} activation and \textit{`AdamOptimizer'} are applied and a model is trained until the tolerance of optimization is $0.0001$ or the maximum $200$ iterations. The neural network of Q-learning has the same architecture of a Neural Network for the Prediction Model (PM).

For the evaluation, this paper utilizes the dataset of three task-oriented, upper-limb stroke rehabilitation exercises recommended by therapists (\textit{`Bring a cup to the mouth', `Switch a light on'}, and \textit{`Move forward a cane'}) \cite{Lee2019LAQ}. Fifteen stroke patients with different level of functional abilities (37 $\pm$ 21 Fugl Meyer Scores) and 11 healthy subjects were participated for data collection with a Kinect v2 sensor  (Microsoft, Redmond, USA) to record the trajectory of body joints at 30 Hz. A patient performed 10 repetitions of each exercise with both affected and unaffected sides. A healthy subject performed 15 repetitions of each exercise with the subject's dominant side. A therapist annotated the entire dataset for implementation.
%and compute the agreement level of a therapist.

In the result so far, the prediction model achieves the good agreement level with therapist's evaluation: 0.8090 - 0.8806 F1-scores. In addition, this paper implements an interface with Kinect SDK and Accord.NET framework \cite{de2014accord}, which can present a patient's exercise motion with joint trajectories, assessment, and real-time audio-based corrective feedback (Figure \ref{fig:web-interface}). A communication channel between an assessment model with python and an interface is implemented with socket programming, which shares the predicted assessment and corrective feedback using identified kinematic variables and user-data.

\section{Conclusion and Future Work}
This paper describes an interactive assessment technique with feature selection that derives personalized motion analysis while generating transparent corrective feedback of motion analysis in terms of real-time audio feedback. The presented interactive assessment achieves good congruence with therapist's evaluation. In future, this interactive technique will be deployed on a socially assistive robot, \cite{shamsuddin2012initial}. In addition, following the study design of \cite{fasola2013socially}, the presented technique will be evaluated on the usefulness of personalized corrective feedback during a post-stroke survivor's rehabilitation session. 

%As this interactive machine learning technique is grounded in statistical principles \cite{van2016deep}, it can be generalized and applied to support other daily activities (e.g. feeding or cooking). The development of a framework that can provide a customizable component (e.g. behaviour analysis, dialogue generator) would facilitate the deployment of elderly care robots. However, significant further work is required to develop elderly care robots with full end-to-end functions (e.g. behaviour analysis, assistance, and companionship) and evaluate their acceptance for elderly people. 

%Ultimately, our goal is the creation of new design guidelines, datasets, algorithmic techniques, and error metrics that can help AI systems realize their enormous potential to benefit PWD, while avoiding the possible pitfalls we have outlined here. 
%We hope this paper provides a research roadmap that can guide AI researchers and practitioners in creating systems that are fair to and effective for PWD. 

\begin{comment}
\section{Acknowledgement}
Thank you to Daniel Siewiorek, Asim Smailagic, Alexandre Bernardino, Sergi Berm{\'u}dez i Badia, Nicola Palmarini, and Peri Tarr for fruitful discussion that helped expand my thinking and research, although they may not agree with all interpretations/conclusions of this paper. The work on monitoring daily activities was done during an internship at IBM Research. All opinion expressed are my own and do not represent any institutional endorsement.



It is questionable how to select kinematic variables for assessment and how well a robot can provide personalized assessment of a patient's rehabilitation exercise. 
If a robot just notifies the output of pre-defined corrective feedback, a patient might consider a robot as not useful and reject to interact with it more \cite{pain2007readiness}. Thus, it is critical to derive a personalized assessment model of a robot for physical therapy sessions. 




In this paper, we present an interactive approach of an assistive robot, which can automatically identify the most salient features to predict the quality of rehabilitation exercises and generate personalized corrective feedback (Figure \ref{fig:approach}). For the development, our approach utilizes the dataset of three upper-limb stroke rehabilitation exercises from 15 post-stroke and 11 healthy subjects that are annotated by therapists. With this dataset, our approach utilizes reinforcement learning \cite{van2016deep} to identify salient features of assessment and predict the quality of motion with a supervised learning algorithm (e.g. Neural Network). When a new patient performs the exercise with patient's unaffected and affected side, our approach dynamically selects user-specific features for assessment and predict the quality of motion with corrective feedback (Figure \ref{fig:interface}).

A new patient can first perform exercise with patient's unaffected side 

When a new patient performs the exercise with patient's unaffected and affected side, 


Once a new patient performs the exercise with patient's unaffected and affected side, the visualization interface of our approach (Figure \ref{fig:web-interface}) shows patient-specific analysis: the predicted quality of motion on three performance components (i.e. \textit{`Range of Motion'}, \

With the selected features and held-out user's unaffected

g to identify salient features of assessmentwith reinforcement learning and predict the quality of motion withsupervised learning algorithms (e.g. Neural Networks). Utilizingidentified features and held-out user data, testing patient’s unaf-fected motions, our approach generates patient-specific analysisthat empowers therapists to understan


dynamically select the most important features for an individual's motion. 



From this dataset, we apply reinforcement learning to identify the most important features for assessment and learn a machine learning model to predict the scores on the exercises of patients. Once a new patient performs the exercise with patient's unaffected and affected side, the visualization interface of our approach (Figure \ref{fig:web-interface}) shows patient-specific analysis: the predicted quality of motion on three performance components (i.e. \textit{`Range of Motion'}, \textit{`Smoothness'}, \textit{`Compensation'}) and the comparison between unaffected and affected sides on the most important kinematic features. Therapists can review this analysis to better understand patient's performance and provide feedback (e.g. feature relevance) to tune a model for personalized rehabilitation assessment.




for the assessment on rehabilitation exercises

of an assistive robot for personalized physical therapy.

that can automatically identify the most salient features for assessment to predict the quality of motion and generate personalized corrective feedback  (Figure \ref{fig:flow-diagram}). 
%Building upon the prior work on creating a rehabilitation assessment system \cite{Lee2019LAQ}, 

\end{comment}
